BlenderAlchemy: Editing 3D Graphics with Vision-Language Models

Graphics design is important for various applications, including movie production and game design. To create a high-quality scene, designers usually need to spend hours in software like Blender, in which they might need to interleave and repeat operations, such as connecting material nodes, hundreds of times. Moreover, slightly different design goals may require completely different sequences, making automation difficult. In this paper, we propose a system that leverages Vision-Language Models (VLMs), like GPT-4V, to intelligently search the design action space to arrive at an answer that can satisfy a user's intent. Specifically, we design a vision-based edit generator and state evaluator to work together to find the correct sequence of actions to achieve the goal. Inspired by the role of visual imagination in the human design process, we supplement the visual reasoning capabilities of VLMs with "imagined" reference images from image-generation models, providing visual grounding of abstract language descriptions. In this paper, we provide empirical evidence suggesting our system can produce simple but tedious Blender editing sequences for tasks such as editing procedural materials and geometry from text and/or reference images, as well as adjusting lighting configurations for product renderings in complex scenes.

==> append_sections/extended_algo.tex <==
\section{Extended BlenderAlchemy Algorithm for Optimizing Multiple Tasks at Once}\label{sec:multiskill_refinement}

As mentioned in the main paper, it's possible to optimize multiple things within the scene at the same time (e.g. lighting and materials, as done for the comet example in the main paper). 
Algorithm \ref{alg:multiskill_refinement} 
outlines how that can be done.

\input{assets/pseudocode/crossdomain_task}




==> figures/ablation_dimensions_samples.tex <==
\begin{figure}[tb]
    \centering
    % placeholder
    \begin{pgfpicture}
      \pgftext{\pgfimage[width=5cm,height=4cm]{methodsoverview.png}}
    \end{pgfpicture}
    \caption{Samples of output materials from different dimensions of our system, for the \textbf{image-based style transfer for material editing} task.}
    \label{fig:ablation_dimensions_samples}
\end{figure}


==> figures/rock_vs_nodegraph.tex <==
\begin{figure}[tb]
    \centering
    % placeholder
    \includegraphics[width=\textwidth]{assets/images/rock_vs_nodegraph.png}
    \caption{\textbf{Procedural materials are complicated.} This is an procedural rock material from the Infinigen~\cite{raistrick2023infinite} library, and its corresponding shader graph on the right. The connection between certain parameters of a single node on the right and the visual changes of the material on the left require trial-and-error and access to visual perception.}
    \label{fig:rock_vs_nodegraph}
\end{figure}

